A corrugated planar-Goubau-line termination for terahertz waves

The planar Goubau line is a promising low-loss metal waveguide for terahertz interconnects. To enable advanced system architectures and multi-port measurements based on planar Goubau lines, there is a strong need for broadband impedance-matched loads, which can be used to absorb the energy and minimize standing waves in a system. In this work, we propose a matched load for planar Goubau lines based on an exponentially-tapered corrugated line, gradually increasing conductor losses while maintaining small reflections. The corrugation density is high enough to increase conductor losses without requiring an auxiliary low-conductivity material, simplifying the fabrication process. A 400-$\mu$m long planar Goubau line load was fabricated on a 10-$\mu$m thick silicon substrate suspended in the air. Electromagnetic simulations of the load show excellent agreement with calibrated reflection measurements in the frequency range 0.5 THz - 1.1 THz. Above the cut-off frequency of around 580 GHz, the measured reflections are much less than -19 dB, below the noise floor of the characterization setup.

==> MySettings.tex <==
\usepackage{amsfonts} 
\usepackage{color}
\usepackage[version=4]{mhchem}
\usepackage{pgfplots}
\usepackage{siunitx}
\usepackage{circuitikz} % For drawing circuits
    \usetikzlibrary{decorations.markings}
    \usepackage{adjustbox}
    \usepackage{adjustbox}
\usepackage{hyperref}
\usepackage{stix}
\usepackage{tikz}
\RequirePackage{tikz} % For Orcid icon

%% ORCID
% Make Orcid icon
\definecolor{lime}{HTML}{A6CE39}
\newcommand{\orcidicon}{%
	\begin{tikzpicture}
	\draw[lime, fill=lime] (0,0) 
		circle [radius=0.16] 
		node[white] {{\fontfamily{qag}\selectfont \tiny ID}};
	\draw[white, fill=white] (-0.0625,0.095) 
		circle [radius=0.007];
	\end{tikzpicture}
	\hspace{-2mm}
}
% Define link and button for each author
\foreach \x in {A, ..., Z}{%
\expandafter\xdef\csname orcid\x\endcsname{\noexpand\href{https://orcid.org/\csname orcidauthor\x\endcsname}{\noexpand\orcidicon}}
}

\usepackage{amsmath}% for double integral symbol in this template
\usepackage{graphicx}% for figures
\usepackage{multirow}% to allow multiple-row elements in tabular environment
\usepackage[none]{hyphenat}% turn off hyphenation to make text extraction and indexing easier
\usepackage{float}% better control of floating figures and tables
\usepackage{subfig}% for subfigures within figures
\captionsetup{font=footnotesize}
\usepackage{dblfloatfix}% fix to allow page-wide floats at bottom of page
\usepackage{siunitx}
\newcommand{\SIadj}[2]{\SI[number-unit-product={\text{-}}]{#1}{#2}}

\usepackage{hyperref}
\usepackage{amsfonts} 

\usepackage{tabularx}
\usepackage{booktabs}



==> Settings.tex <==
% BASIC SETTINGS
\usepackage{caption}
\usepackage{commath}
\usepackage{graphicx, epstopdf}                                                           % Figures
\usepackage{longtable}
\usepackage{mwe}
\setlength{\parskip}{0em}
\usepackage{subcaption}

\usepackage{moreverb}                                                           % List settings
\usepackage{textcomp}                                                           % Fonts, symbols etc.
\usepackage{lmodern}                                                            % Latin modern font
\usepackage{helvet}                                                             % Enables font switching
\usepackage[T1]{fontenc}                                                        % Output settings
%\usepackage[swedish]{babel}                                                    % Language settings
\usepackage[utf8]{inputenc}                                                     % Input settings
\usepackage{amsmath}                                                            % Mathematical expressions (American mathematical society)
\usepackage{amssymb}                                                            % Mathematical symbols (American mathematical society)
\usepackage{subfig}                                                                     % Enables subfigures
\usepackage{listings}                                                           % Enables source code listings
\usepackage{chemfig}                                                    % Chemical structures
\usepackage{siunitx}
\usepackage[a4paper, total={15cm, 23.7cm}]{geometry}
%\usepackage[top=3cm, bottom=3cm,inner=3cm, outer=3cm]{geometry}                 % Page margin lengths                  
\usepackage{eso-pic}                                                            % Create cover page background
\newcommand{\backgroundpic}[3]{
        \put(#1,#2){
        \parbox[b][\paperheight]{\paperwidth}{
        \centering
        \includegraphics[width=0.8\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
       
        
\usepackage{csquotes}
\usepackage{filecontents} 

%

% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)
%\usepackage{color}
\usepackage{comment}
\usepackage{lipsum}
\usepackage{float}
\usepackage{hyperref}
\usepackage{pgfgantt}
\usepackage{etoolbox}
\usepackage{placeins}
\usepackage{xpatch}
\usepackage{siunitx}
\usepackage[super]{nth}
\usepackage{titlesec}
\usepackage{pdfpages}
\usepackage[numbers]{natbib}
\usepackage{units}

%% MATLAB-code fix

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Matlab,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbersf
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}


\epstopdfsetup{outdir=./}
\graphicspath{{./fig/}}

==> include/8_Biography.tex <==

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

% Each author may include a photo and biography in their article, although photos and biographies are often omitted from conference-related articles. Follow these tips for writing your biography. 
% •	If you are an IEEE member, list your status and the corresponding year in parentheses immediately after your name; for example, (M’01–SM’05–F’15) denotes that you became an IEEE Member (M) in 2001, a Senior Member (SM) in 2005, and a Fellow (F) in 2015. 
% •	The first paragraph may contain your place and/or date of birth, followed by your educational background. Degrees should be listed with the type of degree in what field, which institutions, city, state, and country, and the year the degree was earned. Your major field of study should be in lower-case. 
% •	The second paragraph lists military and work experience, with job titles capitalized. Include a location for your current job. List no more than three published books or articles. Include a list of current and previous research interests. In the second paragraph, use the appropriate pronoun and not your last name. 
% •	The third paragraph begins with your title and last name (e.g., Dr. Smith, Prof. Chen) and lists any memberships in professional societies other than IEEE. List any awards and work for IEEE committees and publications. 
% •	If you choose to include a photo, it should be a professional, high-quality headshot. Note that while photos are optional, if they are included, they will be published. 
% Remember, biographies and photos cannot be edited or removed after article publication.


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Juan_photo1.jpg}}]{Juan Cabello-S\'{a}nchez}
(Member, IEEE) was born in Madrid, Spain in 1992. He received a B.Sc. degree in electrical engineering and computer science (2015) from the Polytechnic University of Madrid, Spain; and an M.Sc. degree in electrical engineering (2017) and a PhD degree in terahertz electronics (2022) from the Chalmers University of Technology, Gothenburg, Sweden.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Vlad_photo2.jpg}}]{Vladimir Drakinskiy}
Vladimir Drakinskiy was born in Kurganinsk, Russia, in 1977. He received the Diploma in physics and informatics (Hons.) from the Armavir State Pedagogical Institute, Armavir, Russia, in 2000.

From 2000 to 2003, he was a Junior Research Assistant with the Physics Department, Moscow State Pedagogical University. Since 2003, he has been with the Department of Microtechnology and Nanoscience (MC2), Chalmers University of Technology, Gothenburg, Sweden. From 2003 to 2005, he was responsible for the mixer chip fabrication for the Herschel Space Observatory. Since 2008, he has been a Research Engineer with the MC2, Chalmers University of Technology. He is currently responsible for the terahertz Schottky diode  rocess line at MC2, Chalmers University of Technology. His research interests include microfabrication and nanofabrication techniques, detectors for submillimeter and THz ranges, and superconducting thin films.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Jan_photo3.jpg}}]{Jan Stake}
(S' 95--M' 00--SM' 06) was born in Uddevalla, Sweden, in 1971. He received the M.Sc. degree in electrical engineering and the Ph.D. degree in microwave electronics from the Chalmers University of Technology, Goteborg, Sweden, in 1994 and 1999, respectively.

In 1997 he was a Research Assistant with the University of Virginia, Charlottesville, USA. From 1999 to 2001, he was a Research Fellow with the Millimetre Wave Group at the Rutherford Appleton Laboratory, Didcot, UK. He then joined Saab Combitech Systems AB, as a Senior RF/microwave Engineer, until 2003. From 2000 to 2006, he held different academic positions with Chalmers University of Technology and, from 2003-2006, was also Head of the Nanofabrication Laboratory, Department of Microtechnology and Nanoscience (MC2). During 2007, he was a Visiting Professor with the Submillimeter Wave Advanced Technology (SWAT) Group at Caltech/JPL, Pasadena, USA. In 2020, he was a Visiting Professor at TU Delft. He is currently Professor and Head of the Terahertz and Millimetre Wave Laboratory, Chalmers University of Technology, Sweden. He is also cofounder of Wasa Millimeter Wave AB, Göteborg, Sweden. His research involves graphene electronics, high-frequency semiconductor devices, THz electronics, submillimeter wave measurement techniques, and terahertz systems.

Prof. Stake served as Editor-in-Chief for the IEEE TRANSACTIONS ON TERAHERTZ SCIENCE AND TECHNOLOGY between 2016-2018 and topical editor between 2012-2015.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Helena_photo4.jpg}}]{Helena Rodilla}
(M' 16--SM' 20) was born in Salamanca, Spain, in 1982. She received the B.S. and Ph.D. degrees in Physics from the University of Salamanca, Salamanca, Spain, in 2006 and 2010, respectively.

From 2006 to 2010, she was with the Electronics Group, Department of Applied Physics, University of Salamanca, Spain, where her research interest was semiconductor physics. From 2011 to 2013 she was Postdoctoral Researcher with the Microwave Electronics Laboratory, Department of Microtechnology and Nanoscience (MC2), Chalmers University of Technology, Gothenburg, Sweden, where she worked on very low-noise InP HEMTs for cryogenic low noise amplifiers. Since 2013 she has been with the Terahertz and Millimetre Wave Laboratory, MC2, Chalmers University of Technology, Gothenburg, Sweden, where she became Associate Professor in 2020. Her current research interests include the use of millimeter wave and terahertz technology in life science applications, sensing and on-wafer terahertz measurements.

\end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> include/Papers_to_cite.tex <==
\section{Papers to cite}

\begin{itemize} 
    \item "Terahertz Microfluidic Metamaterial Biosensor for Tiny Volume Liquid Samples" \cite{Zhang2019a}
\end{itemize}

